Robust Ranking Explanations

Robust explanations of machine learning models are critical to establish human trust in the models. Due to limited cognition capability, most humans can only interpret the top few salient features. It is critical to make top salient features robust to adversarial attacks, especially those against the more vulnerable gradient-based explanations. Existing defense measures robustness using $\ell_p$-norms, which have weaker protection power. We define explanation thickness for measuring salient features ranking stability, and derive tractable surrogate bounds of the thickness to design the \textit{R2ET} algorithm to efficiently maximize the thickness and anchor top salient features. Theoretically, we prove a connection between R2ET and adversarial training. Experiments with a wide spectrum of network architectures and data modalities, including brain networks, demonstrate that R2ET attains higher explanation robustness under stealthy attacks while retaining accuracy.

==> addtional_experiment.tex <==
\newpage
\section{Additional Experimental Results}
To address the reviewers' comments and suggestions, 
we replenish some experimental results in this section.
Specifically, 
\begin{itemize}[leftmargin=*]
    \item We consider Adversarial Training (AT) as a new baseline, 
    and compare it with R2ET and other training methods.
    \item We try two more gradient-based methods as explanation methods, 
    SmoothGrad (SG) \cite{smilkov2017smoothgrad} and Integrated Gradients (IG) \cite{sundararajan2017axiomatic}, 
    to extract explanations for all the models, see Table \ref{tab:SG_IG}.
    \item We evaluate the faithfulness of gradient-based explanation methods on the models trained by different methods, see Table \ref{tab:faithfulness}.
    \item We also report the model-level thickness of all the models, see Table \ref{tab:thickess_patk}. 
\end{itemize}

\subsection{Adversarial Training}
We train the model following a minimization-maximization approach \cite{huang2015learning,shaham2018understanding} that
\begin{equation*}
\begin{aligned}
    \min_{f} &
    \sum_{(\mathbf{x},y)\in(\mathcal{X}_T,\mathcal{Y}_T)}
    (\mathcal{L}_{cls} (f;\mathbf{x}+\delta^\ast, y)), \\
    \textnormal{s.t.} & \quad
    \delta^\ast = \argmax_\delta - \sum_{i=1}^k \sum_{j=k+1}^n
    h(\mathbf{x}+\delta, i,j).
\end{aligned}
\end{equation*}

\noindent \textbf{Experimental Results.}
Concerning the classification performance,
AT models on most datasets have high clean AUC (drops not more than 1\% compared with the vanilla model). 
Specifically, 
for Adult, Bank, COMPAS, MNIST, ADHD and BP,
the AT models achieve cAUC of 0.87, 0.64, 0.82, 0.99,
0.73, and 0.64.
Correspondingly, 
the adversarial AUC (under ERAttack) is 0.87, 0.65, 0.81, 0.99, 0.73, and 0.63.
The AUC performance of other models concerning the classification task has already been disclosed in Sec. \ref{sec:supp_cauc} and Sec. \ref{sec:acc_robust_trade_off}.
We will report the performance of AT models concerning other metrics in the following.


\subsection{SG and IG as explanation methods}
Instead of using the simple gradient of the models with respect to inputs as the explanations, 
we here adopt two other gradient-based explanation methods, 
including SmoothGrad (SG) \cite{smilkov2017smoothgrad} and Integrated Gradients (IG) \cite{sundararajan2017axiomatic}.

SG takes random samples in a small neighborhood of input $\mathbf{x}$,
and computes the average of the saliency maps for these random samples as the final results for $\mathbf{x}$. 
Particularly,
we consider adding a Gaussian noise obeying $\mathcal{N}(0, \sigma^2I)$ to the original inputs, 
\begin{equation*}
    \mathcal{I}_{SG}(\mathbf{x}) = \frac{1}{M}\sum_i \mathcal{I}(\mathbf{x}+\delta), 
    \quad \textnormal{s.t.} \quad
    \delta \sim \mathcal{N}(0,\sigma^2I).
\end{equation*}
$M$ is the number of neighboring samples around $\mathbf{x}$.
In practice, 
we set $M$=50 for all datasets, 
and $\sigma^2=0.5, 25.5^2 \textnormal{ and } 0.01$ for tabular, image and graph datasets, respectively.

IG is defined as the integration of the saliency maps along a path from a reference point $\mathbf{x}^0$ to input $\mathbf{x}$.
Formally,
\begin{equation*}
    \mathcal{I}_{IG}(\mathbf{x}) = 
    (\mathbf{x}-\mathbf{x}^0)\int_{\alpha=0}^1 
    \frac{\partial f(\mathbf{x}^0+\alpha (\mathbf{x}-\mathbf{x}^0))}{\partial \mathbf{x}} d\alpha.
\end{equation*}
In practice, we set the reference point $\mathbf{x}^0$ as the all-zero vector, 
and approximate the integration by interpolating 100 samples between $\mathbf{x}^0$ and $\mathbf{x}$.

\noindent \textbf{Experimental Results.}
We extract explanations by Simple Gradient, SG and IG, respectively,
and report the P@$k$ metric of the models under ERAttack in Table \ref{tab:SG_IG}.
Overall, SG and IG generate more robust explanations for most of models under attacks.
Moreover, 
the relative performance rankings among different training methods remain the same, 
no matter the simple gradient, SG or IG is adopted as the explanation methods.
Especially,
R2ET and its variants achieve the best performance in most datasets and are compatible with other gradient-based explanation methods, such as SG and IG, for even better robustness.

Since R2ET and other baselines are \textit{training} methods for better explanation ranking robustness,
we do NOT encourage comparing R2ET with SG, which is an \textit{explanation} method.
Specifically, 
both training method and explanation method change if comparing (Vanilla + SG) with (R2ET + Simple Gradient).
Instead, we compare (Vanilla + Simple Gradient) with (R2ET + Simple Gradient) to investigate the superiority of training methods, 
or to compare (R2ET + IG) with (R2ET + SG) to explore the stability of the explanation methods.


\begin{table*}[!tb]
\caption{The P@$k$ (shown in percentage) of different models under ERAttack, $k=8$ for the first three dataset and $k=50$ for the rest.
We report P@$k$ for \textbf{Simple Gradient} (from Table \ref{tab:comprehensive_result}), \textbf{SG} and \textbf{IG}, respectively.
}
\centering
\begin{tabular}{ c || c c c}
\toprule
\textbf{Method} & Adult & Bank
& COMPAS \\
% & MNIST & ADHD & BP \\
\midrule
Vanilla & 
87.6 / 94.0 / \textbf{71.8} & 83.0 / 90.0 / 88.1 & 84.2 / 92.9 / 94.7 
% & 59.0 / 67.9 / 82.8 & 45.5 /  & 69.4 / 
\\
WD &
91.7 / 97.3 / 55.5 & 82.4 / 91.3 / 85.7 & 87.7 / 97.4 / 99.1 
% &
% 59.1 / 68.3 / 83.0 & 47.6 / & 69.4 / 
\\
SP & 
\underline{97.4} / 95.3 / \underline{63.9} & 95.4 / 96.7 / \underline{99.9} & \textbf{99.5} / \textbf{100.0} / \textbf{100.0} 
% &
% 62.9 / 69.0 / 85.4 & 42.5 /  & 68.7 / 
\\
Est-H & 
87.1 / 93.1 / 61.5 & 78.4 / 87.3 / 82.4 & 82.6 / 89.9 / 89.9 
% &
% 85.2 / 87.9 / 89.5 & 58.2 / & \textbf{75.0} /
\\
Exact-H & 
89.6 / 95.8 / 62.1 & 81.9 / 89.7 / 90.0 & 77.2 / 91.6 / 90.8 
% &
% - / - / - & - / - / - & - / - / -
\\
SSR & 
91.2 / 93.0 / 62.5 & 76.3 / 84.9 / 85.4 & 82.1 / 96.2 / \underline{99.5} 
% &
% - / - / - & - / - / - & - / - / -
\\
AT & 68.4 / 76.6 / 60.0 & 80.0 / 85.9 / 82.6 & 84.2 / 85.9 / 82.4 
% & 56.0 / 61.5 / 79.3
\\
\midrule
$\textnormal{R2ET}_{\backslash H}$ & 
\textbf{97.5} / 97.5 / 57.3 & \textbf{100.0} / \textbf{100.0} / \textbf{100.0} & 91.0 / 96.6 / 93.6 
% &
% 82.8 / 87.1 / 89.0 & 60.7 / & 70.9 / 
\\
R2ET-$\textnormal{mm}_{\backslash H}$ &
93.5 / 97.4 / 55.9 & \underline{95.8} / \underline{97.0} / 96.3 & \underline{95.3} / 99.1 / 95.5 
% &
% 81.6 / 86.8 / 88.7 & \underline{64.2} /  & 72.4 / 
\\
\midrule
R2ET & 
92.1 / \textbf{99.3} / 54.0 & 80.4 / 88.9 / 84.4 & 92.0 / \underline{99.7} / \textbf{100.0} 
% &
% \textbf{85.7} /  & \textbf{73.8} /  & 71.5 / 
\\
R2ET-mm &
87.8 / \underline{98.6} / 54.2 & 75.1 / 85.1 / 80.3 & 82.1 / 93.5 / \underline{99.5} 
% &
% \underline{85.3} / 88.3 / 90.1 & 60.1 /  & \underline{73.8} / 
\\
\bottomrule
\end{tabular}
\begin{tabular}{ c || c | c c}
\toprule
\textbf{Method} & MNIST & ADHD & BP \\
\midrule
Vanilla & 
59.0 / 67.9 / 82.8 
& 45.5 / 39.0 / 56.9 
& 69.4 / 59.6 / 60.8
\\
WD &
59.1 / 68.3 / 83.0 
& 47.6 / 42.3 / 57.2
& 69.4 / 61.8 / 63.9
\\
SP & 
62.9 / 69.0 / 85.4 
& 42.5 / 36.9 / 54.9 
& 68.7 / 58.6 / 60.5
\\
Est-H & 
85.2 / 87.9 / 89.5 
& 58.2 / 48.9 / 54.7
& \textbf{75.0} / 63.0 / 58.5
\\
Exact-H & 
- / - / - & - / - / - & - / - / -
\\
SSR & 
- / - / - & - / - / - & - / - / -
\\
AT & 
56.0 / 61.5 / 79.3
& 59.4 / 41.2 / 43.0
& 72.0 / 56.7 / 54.4
\\
\midrule
$\textnormal{R2ET}_{\backslash H}$ & 
82.8 / 87.1 / 89.0 
& 60.7 / 56.9 / \underline{61.9}
& 70.9 / 64.2 / \textbf{66.0}
\\
R2ET-$\textnormal{mm}_{\backslash H}$ &
81.6 / 86.8 / 88.7 
& \underline{64.2} / \underline{59.5} / \underline{61.9}
& 72.4 / \underline{65.5} / 64.1
\\
\midrule
R2ET & 
\textbf{85.7} / \textbf{88.5} / \textbf{90.4} 
& \textbf{71.6} / \textbf{67.2} / \textbf{65.8}
& 71.5 / 64.0 / \underline{65.0}
\\
R2ET-mm &
\underline{85.3} / \underline{88.3} / \underline{90.1} 
& 58.8 / 50.1 / 51.4
& \underline{73.8} / \textbf{65.6} / 63.9
\\
\bottomrule
\end{tabular}
\label{tab:SG_IG}
\end{table*}

\subsection{Faithfulness of explanations on different models}

We consider three widely adopted metrics to evaluate the faithfulness of models.
\begin{itemize}[leftmargin=*]
    \item \textbf{Decision Flip - Fraction of Tokens (DFFOT)} \cite{serrano2019attention} measures the minimum fraction of important features to be removed to flip the prediction.
    A \textit{lower} DFFOT indicates a more faithful explanation.
    Formally,
    \begin{equation*}
    \textnormal{DFFOT} = \min_k \frac{k}{n}, 
        \quad 
        \textnormal{s.t.}
        \quad
        \argmax_c f(x)_c \neq \argmax_c f(x_{[\backslash k]})_c,
    \end{equation*}
    where $n$ is the number of features of the input, and $x_{[\backslash k]}$ is the perturbed input whose  top-$k$ important features being removed.
    
    \item \textbf{Comprehensiveness (COMP)} \cite{deyoung2019eraser} 
    measures the changes of predictions before and after removing the most important features.
    A \textit{higher} COMP means a more faithful explanation. Formally,
    \begin{equation*}
        \textnormal{COMP} = \frac{1}{\|K\|} \sum_{k\in K} |f(x)_c - f(x_{[\backslash k]})_c |,
    \end{equation*}
    where $K={1,\dots,n}$ for tabular data, 
    and  $K=\{1\% *n, 5\% *n, 10\% *n, 20\% *n, 50\% *n\}$ for images and graphs.
    
    \item \textbf{Sufficiency (SUFF)} \cite{deyoung2019eraser}
    measures the change of predictions if only the important tokens are preserved.
    A \textit{lower} SUFF means a more faithful explanation.
    Formally,
    \begin{equation*}
        \textnormal{SUFF} = \frac{1}{\|K\|} \sum_{k\in K} |f(x)_c - f(x_{[k]})_c |,
    \end{equation*}
    where $x_{[k]}$ is the perturbed input with only top-$k$ important features, 
    and $K$ is set the same as the one for COMP.
\end{itemize}

\textbf{Experimental Results.}
The results can be found in Table \ref{tab:faithfulness}.

\begin{table*}[!tb]
\caption{Faithfulness of explanations evaluated by DFFOT ($\downarrow$) / COMP ($\uparrow$) / SUFF ($\downarrow$).}
\centering
\small
\begin{tabular}{ c || c c c | c | c c}
\toprule
\textbf{Method} & Adult & Bank
& COMPAS & MNIST & ADHD & BP \\
\midrule
Vanilla 
& 0.24 / 0.43 / 0.18
& 0.23 / 0.14 / 0.04
& \textbf{0.17} / 0.37 / \underline{0.14} 
& 0.37 / 0.16 / 0.23
& 0.51 / 0.05 / 0.28
& 0.40 / \underline{0.06} / 0.29
\\
WD 
& 0.45 / 0.47 / 0.23
& 0.36 / 0.27 / 0.07 
& 0.29 / 0.41 / 0.18
& 0.37 / 0.16 / 0.22
& 0.49 / 0.06 / 0.27
& \textbf{0.35} / 0.05 / 0.33
\\
SP 
& 0.43 / 0.47 / 0.25
& 0.35 / 0.31 / 0.07 
& 0.29 / \textbf{0.45} / 0.18
& 0.38 / 0.15 / 0.22
& \textbf{0.30} / 0.10 / 0.34
& \underline{0.38} / \underline{0.06} / 0.30
\\
Est-H 
& 0.44 / 0.44 / 0.24
& 0.18 / 0.21 / 0.06
& 0.27 / 0.42 / 0.17
& 0.23 / \underline{0.24} / \textbf{0.18}
& 0.59 / 0.04 / \underline{0.26}
& 0.45 / 0.05 / \textbf{0.24}
\\
Exact-H 
& 0.43 / 0.46 / 0.23
& 0.19 / 0.14 / 0.04
& 0.30 / 0.40 / 0.18
& - / - / -
& - / - / -
& - / - / -
\\
SSR
& 0.54 / 0.39 / 0.21
& 0.46 / 0.04 / \textbf{0.01}
& 0.32 / 0.43 / 0.18
& - / - / -
& - / - / -
& - / - / -
\\
AT 
& \underline{0.16} / 0.14 / \textbf{0.08}
& 0.19 / 0.10 / \underline{0.03}
& \underline{0.24} / 0.10 / \textbf{0.07} 
& 0.40 / 0.12 / 0.28
& \underline{0.35} / 0.10 / \underline{0.26}
& 0.46 / \underline{0.06} / \underline{0.25}
\\
\midrule
$\textnormal{R2ET}_{\backslash H}$ 
& \textbf{0.13} / \textbf{0.50} / \underline{0.14}
& 0.34 / \underline{0.32} / 0.10
& \textbf{0.17} / 0.40 / 0.17
& 0.23 / 0.22 / \underline{0.19}
& 0.38 / \underline{0.13} / 0.37
& 0.43 / \textbf{0.07} / 0.29
\\
R2ET-$\textnormal{mm}_{\backslash H}$ 
& 0.42 / 0.47 / 0.22
& 0.34 / \textbf{0.41} / 0.14
& 0.25 / 0.42 / 0.17
& 0.25 / 0.22 / 0.21
& 0.37 / \textbf{0.17} / 0.37
& 0.42 / \textbf{0.07} / 0.29
\\
\midrule
R2ET 
& 0.32 / 0.46 / 0.19
& \textbf{0.11} / 0.24 / 0.07
& 0.27 / 0.39 / 0.17
& \textbf{0.18} / \textbf{0.26} / 0.23
& 0.48 / 0.12 / \underline{0.26}
& 0.42 / \textbf{0.07} / 0.29
\\
R2ET-mm 
& 0.38 / \underline{0.48} / 0.20
& \underline{0.12} / 0.21 / 0.08
& 0.28 / \underline{0.44} / 0.15
& \underline{0.19} / \textbf{0.26} / 0.22
& 0.50 / 0.04 / \textbf{0.25}
& 0.45 / 0.05 / 0.29

\\
\bottomrule
\end{tabular}
\label{tab:faithfulness}
\end{table*}


\subsection{Thickness of models}
Per the request of the reviewers, 
to support the claims in Sec. \ref{sec:relation_thickness_other_metric} that models with larger thickness should have better ranking robustness under attacks.
We report the model-level thickness for all the models in Table \ref{tab:faithfulness}.
The model-level thickness is defined as the average thickness, 
defined in Eq. (\ref{eq:topk_rank_thick}), 
of all the samples.
To explore the correlation between P@$k$ metrics in Table \ref{tab:comprehensive_result} and the thickness,
we show these two measurements in one unified Table \ref{tab:thickess_patk}.
Clearly,
the models with high P@$k$ performance usually have a relatively large thickness as well,
and vice versa.

\begin{table*}[!tb]
\caption{\small The \textbf{P}@\boldsymbol{$k$} (shown in percentage) of different robust models (rows) under ERAttack and the values of \textbf{thickness}.}
\centering
% \small
\begin{tabular}{ c || c c c | c | c c}
\toprule
\textbf{Method} & Adult & Bank
& COMPAS & MNIST & ADHD & BP \\
\midrule
Vanilla & 
87.6 / 0.9889 & 83.0 / 0.9692  & 84.2 / 0.9533 &
59.0 / 0.9725 
& 45.5 / 0.9261 
& 69.4 / 0.9282 
\\
WD &
91.7 / 0.9960  & 82.4 / 0.9568 & 87.7 / 0.9769 &
59.1 / 0.9732 
& 47.6 / 0.9343 
& 69.4 / 0.9298 
\\
SP & 
\underline{97.4} / \underline{0.9983} & 95.4 / \underline{0.9978} & \textbf{99.5} / \textbf{0.9999} &
62.9 / 0.9771 
& 42.5 / 0.9316
& 68.7 / 0.9300 
\\
Est-H & 
87.1 / 0.9875 & 78.4 / 0.9583 & 82.6 / 0.9557  &
85.2 / \underline{0.9948} 
& 58.2 / 0.9578
& \textbf{75.0} / \textbf{0.9356} 
\\
Exact-H & 
89.6 / 0.9932 & 81.9 / 0.9521 & 77.2 / 0.9382 &
- / - & - / - & - / -
\\
SSR & 91.2 / 0.9934 & 76.3 / 0.9370 & 82.1 / 0.9549 &
- / - & - / - & - / - 
\\
AT & 68.4 / 0.9372 & 80.0 / 0.9473 &  84.2 / 0.9168 & 56.0 / 0.9639
& 59.4 / 0.9597
& 72.0 / \underline{0.9342} 
\\
\midrule
$\textnormal{R2ET}_{\backslash H}$ & 
\textbf{97.5} / \textbf{0.9989}  & \textbf{100.0} / \textbf{1.0000} & 91.0 / 0.9727 &
82.8 / \textbf{0.9949} 
& 60.7 / 0.9588
& 70.9 / 0.9271 
\\
R2ET-$\textnormal{mm}_{\backslash H}$ &
93.5 / 0.9963 & \underline{95.8} / 0.9874 & \underline{95.3} / \underline{0.9906} &
81.6 / 0.9942 
& \underline{64.2} / \underline{0.9622}
& 72.4 / \underline{0.9342} 
\\
\midrule
R2ET & 
92.1 / 0.9970 & 80.4 / 0.9344 & 92.0 / 0.9865 &
\textbf{85.7} / \textbf{0.9949} 
& \textbf{71.6} / \textbf{0.9731}
 & 71.5 / 0.9296 
\\
R2ET-mm &
87.8 / 0.9943 & 75.1 / 0.9102 & 82.1 / 0.9544 &
\underline{85.3} / \underline{0.9948} 
& 58.8 / 0.9588
& \underline{73.8} / \textbf{0.9356} 
\\
\bottomrule
\end{tabular}
\label{tab:thickess_patk}
\end{table*}


==> analysis.tex <==
\section{Analysis}
\label{sec:analysis}
We provide theoretical analyses to understand how maximizing the thickness can improve explanation robustness under adversarial attacks.
Different from prior work, we characterize the worst-case complexity of explanation robustness using constrained multi-objective optimization.

\noindent\textbf{Threat model.}
Given the model $f$, an input $\mathbf{x}$, and an initial feature ranking, 
% we provide an upper bound of the number of iterations for the attacker to
the attacker aims to swap the ranking of any pair of a salient feature $i$ and a non-salient feature $j$,
so that the gap $h(\mathbf{x}, i,j)$ defined in Eq. (\ref{eq:defense_thick}) becomes negative.
The attacker needs to constrain itself to neither change the input $\bx$ nor the predictions $f(\bx)$ significantly for stealthiness.
% Figure~\ref{fig:attack_performance} in the Appendix shows that imposing these constraints can make attacking the explanation more challenging.  
Imposing these constraints can make attacking the explanation more challenging.  
We assume that the attacker has access to the parameters and architecture of the model $f$ to conduct gradient-based white-box attacks, which is stronger than black-box attacks,
as we don't have the sign of obfuscated gradients~\cite{athalye2018obfuscated} (see Figure~\ref{fig:correlation_manipulation_epoch}).

% \subsection{Maximizing ranking thickness increases robustness}
% \label{sec:analysis_maximizing_ranking_thickness}
% motivation of the MOO formulation and analysis
\noindent\textbf{Optimization problem for the attack}.
Each $h(\bx, i,j )$ is an objective function for the attacker,
who
however does not know which objective is the easiest to attack.
Furthermore, attacking one objective can make another easier or harder to attack due to their dependency on the same model $f$ and the input $\bx$.
As a result, an attack against a specific target feature pair does not reveal the true robustness of the feature ranking. 
We quantify the hardness of a successful attack (equivalently, explanation robustness) by an upper bound on the number of iterations for the attacker to flip the \textit{first} (unknown) feature pair.
The longer it takes to flip the first pair, 
the more robust the explanations of $f(\bx)$.
Formally, for any given initial input $\bx^{(0)}$ ($(k)$ in the superscript means the $k$-th attacking iteration),
the attacker needs to iteratively manipulate $\bx$ to reduce the gaps $h(\bx, i, j)$ for all $i\in\{1,\dots,k\}$ and $j\in\{k+1,\dots, n\}$ packed in a vector objective function:

MOO-Attack($\bx$,$\epsilon$):
\begin{equation}
    \left\{
    \begin{array}{cl}
        \min_{\bx}
    	~~ & [h_1(\bx),\dots, h_\ell(\bx),\dots, h_m(\bx)],\\
    	\mbox{s.t.} ~~ &
        \|f(\bx) -  f(\bx^{(0)})\| \leq \epsilon,
    \end{array}
    \label{eq:attack_moo}
    \right.
\end{equation}
with $h_\ell(\bx) \defeq h(\bx, i, j)$, with $\ell$ indexing the $(i,j)$ pairs.

\textit{Comments:}
(i) the scalar function $\sum_i \sum_j h(\bx, i, j)$ is not suitable for theoretical analyses,
since at a stationary point of the sum,
there can be no pair of features flipped.
Minimizing multiple objectives simultaneously allows us to determine when the first pair of features is flipped and gives a pessimistic bound for the defender (and thus an optimistic bound for the attacker).
Empirically, minimizing $\sum_i \sum_j h(\bx, i, j)$ suffices to attack some explanations.
% the vector optimization allows analyzing the convergence from an arbitrary starting point to \textit{any} Pareto optimal solution where reducing the gap for one $(i,j)$ pair necessarily increases the gap of at least another pair, that is, it is impossible to reduce all gaps simultaneously.
(ii) We could have adopted the Pareto criticality for convergence analysis as in~\cite{Fliege2016}, but a Pareto critical point indicates that no critical direction (moving in which does not violate the constraint) leads to a joint descent in \textit{all} objectives,
rather than that an objective function $h_\ell$ has been sufficiently minimized.
(iii) Different from the local convergence results in~\cite{Fliege2000}, we provide a global rate of convergence that justifies thickness maximization, and different from the unconstrained case in~\cite{Fliege2019}, we constrain the amount of changes in $\bx$ and $f(\bx)$.

On the high level, we propose a trust-region method  Algorithm~\ref{alg:moo_attack} in the Appendix to solve MOO-Attack($\bx$, $\epsilon$).
If the algorithm reaches a critical point (where at least one objective function cannot be reduced)
without flipping any pair of features,
the objective function(s) that cannot be further reduced will be removed from objective vector of MOO-Attack($\bx$, $\epsilon$)
and Algorithm~\ref{alg:moo_attack} will run on the remaining objectives.
Since it takes a bounded number of iterations to reach a critical point (Theorem~\ref{thm:attack_moo}) and the objective functions are monotonically decreasing after each run of the algorithm (Lemma~\ref{lem:suff_reduction_target}),
the number of iterations for an attacker to flip a pair of features, or to claim that the attack fails, is bounded by $\lceil m(h_{\textnormal{up}}-h_{\textnormal{low}})\frac{\kappa}{\epsilon^2}\rceil$,
where
$m$ is the number of objectives,
$h_{\textnormal{up}}-h_{\textnormal{low}}$ is the distance between the maximum of any $h_\ell$ and the minimum of any $h_\ell$, $\kappa$ is a constant depending the parameters of the trust-region method and the smoothness of the objective and constraint functions, and $\epsilon$ is the tolerance of optimization accuracy.

Technically, 
for each objective function $h_\ell(\bx)$ and a scalar target $t\in\mathbb{R}$,
define the merit function $\phi_\ell$ that combines the $\ell$-th objective and the constraint in Eq. (\ref{eq:attack_moo}):
\begin{equation}
\label{eq:merit_func}
    \phi_\ell(x,t)\defeq \|f(\bx)\| + |h_\ell(\bx)-t_\ell|.
\end{equation}
Lemma~\ref{lem:invariant} in the Appendix shows these merit functions will remain small while the targets $t_\ell$, and thus $h_\ell$, can be jointly minimized.
As an approximating model for the trust-region method,
define the linearization of $\phi(\bx, t)$ as
\begin{equation}
\label{eq:merit_func_linear}
    l_{\phi_{\ell}}(\bx, t, \mathbf{d})
    = \|f(\bx)+J(\bx)^\top \mathbf{d}\| + |h_\ell(\bx)+g_\ell(\bx)^\top \mathbf{d}-t|,\nonumber
\end{equation}
where $J(\bx)$ is the Jacobian of $f$ at $\bx$ and $g_\ell(\bx)$ is the gradient of $h_\ell$ at $\bx$.
The maximal reduction in $l_{\phi_{\ell}}(\bx, t, 0)$ within a radius of $\Delta>0$ at $\bx$ is
\begin{equation}
    \chi_\ell(\bx, t)\defeq l_{\phi_{\ell}}(\bx, t, 0) - \min_{\mathbf{d}:\|\mathbf{d}\|\leq \Delta} l_{\phi_{\ell}}(\bx, t, \mathbf{d}).
\end{equation}
When $\chi_\ell(\bx, t)=0$ (or $\leq \epsilon$), $\bx$ is a critical (approximately critical) point of $\phi_\ell$.

The core of Algorithm~\ref{alg:moo_attack} is the following optimization problem, TR-MOO$(\bx,\Delta)$,
whose optimal solution provides a descent direction $\mathbf{d}$
for all $l_{\phi_\ell}$ (not $h_\ell$ or $\phi_\ell$):
% The descent direction $\mathbf{d}$ is found by solving the quadratic programming 
\begin{equation}
    \left\{
    \begin{array}{cl}
         \min_{\alpha,\mathbf{d}} & \alpha   \\
        \textnormal{s.t.} & l_{\phi_{\ell}}(\bx,t,\mathbf{d})\leq \alpha, \ell=1,\dots, m,\\
        & \|\mathbf{d}\|\leq \Delta.
    \end{array}
    \nonumber
    \right.
\end{equation}
where $\alpha$ is the minimal amount of descent and $\Delta$ is the current radius of search for $\mathbf{d}$.
With details in the Appendix, we show the following convergence result:
\begin{theorem}
\label{thm:attack_moo}
Suppose assumptions H.1-H.3 in the Appendix hold.
Then Algorithm~\ref{alg:moo_attack} generates an $\epsilon$-first-order critical point for problem Eq. (\ref{eq:moo_attack}) in at most
\begin{equation}
    \Bigl\lceil\left(h_{\textnormal{up}}-h_{\textnormal{low}}\right)\frac{\kappa}{\epsilon^2}\Bigr\rceil
\end{equation}
iterations, where $\kappa$ is a constant independent of $\epsilon$ but depending on the parameters $\gamma$ and $\eta$ of the trust-region method, and the global Lipschitz constants $L_J$ of the Jacobian $J$ and $L_{g_\ell}$ of the gradients $g_\ell$.
\end{theorem}

% For the attacker to make descent in all objectives, 
% it needs to search a small enough step size $\eta$, 
% To make descent in all objectives, 
% the attack searches a small enough step size $\eta$, 
% such that
% \begin{equation}
%     \label{eq:sufficient_descent}
%     F_k(\bx+\eta \mathbf{d})-F_k(\bx) \leq \beta \eta \nabla F_k(\bx)^\top \mathbf{d},\hspace{.1in} \forall k=1,\dots, m.
% \end{equation}

% The algorithm guarantees convergence of the attack,
% since at each step a minimal descent $\beta_{\min} \eta \alpha$, $\beta_{\min} > 0$ for any $k=1,\dots, m$, is guaranteed, as shown by the following lemma and theorem.
% \begin{lemma}
% \label{lem:descent}
%     Assume that each $\nabla F_k$ is Lipschitz with Lipschitz constant $L_k$.
%     Let $L_{\max}=\max\{L_1,\dots, L_m\}$.
%     Then there exists some sufficiently small $\eta > \eta_{\min} =\min\{(1-\beta)/L_{\max},1\}$ to make descents in all $m$ objectives.
% \end{lemma}

% \begin{theorem}
% \label{thm:convergence}
%     Let $F^{\min}$ be the smallest value of any $F_k$ and $F^{\max}=\max_k F_k(\bx^{(0)})$.
%     Then the iterate $\bx^{(t+1)}=\bx^{(t)}-\eta^{(t)} \mathbf{d}^{(t)}$ will converge in the sense that $\min_{1\leq \tau\leq t} \|\mathbf{d}^{(\tau)}\|\to 0$ at the rate of $1/\sqrt{t}$.
% \end{theorem}
% $F^{\text{min}}$ is the smallest possible value of the thickness $h(\bx, i,j)$ for any feature pair $(i,j)$, the goal that the attacker aims to attain,
% and $F^{\max}$ represents the initial thickness the attacker starts to attack.
% Intuitively, when $t$ is sufficiently large, one will eventually encounter a sufficiently small $\mathbf{d}^{(\tau)}$ as an indicator to stop the iterates at $\tau$ when the algorithm has found a (local) Pareto optimum.

% Iterative attacks algorithms with constraints, such as constraining the predictions of $f$ to be unchanged, can be analyzed in a similar way,
% with turning the constraints into additional objective functions~\cite{Fliege2016}.

==> checklist.tex <==
% \newpage
\section{Reproducibility Checklist}

\begin{enumerate}[leftmargin=*]
    \item This paper
    \begin{enumerate}
        \item Includes a conceptual outline and/or pseudocode description of AI methods introduced. [Yes, see Eq. (\ref{eq:defense_thick}) in Sec. \ref{sec:ranking_thickness_defense}.]
        \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results. [Yes.]
        \item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper. [Yes.]
    \end{enumerate}
    
    \item Does this paper make theoretical contributions? [Yes.]
    \begin{enumerate}
        \item All assumptions and restrictions are stated clearly and formally. [Yes, see Sec. \ref{sec:thickness_whole_section}, \ref{sec:analysis}, and Appendix \ref{sec:appendix-proof}.]
        \item All novel claims are stated formally (e.g., in theorem statements). [Yes, see discussion on Sec. \ref{sec:ranking_thickness_defense} and \ref{sec:analysis}.]
        \item Proofs of all novel claims are included. 
        [Yes, see Appendix \ref{sec:appendix-proof}.]
        \item Proof sketches or intuitions are given for complex and/or novel results. [Yes, see discussion on Sec. \ref{sec:ranking_thickness_defense}.]
        \item Appropriate citations to theoretical tools used are given. 
        [Yes.]
        \item All theoretical claims are demonstrated empirically to hold. [Yes, see Sec. \ref{sec:experiemnt_whole_section} and Appendix \ref{sec:append_experiments}.]
        \item All experimental code used to eliminate or disprove claims is included. [NA. Experimental code will be released after publication, while the complete experimental results are shown in Sec. \ref{sec:experiemnt_whole_section} and Appendix \ref{sec:append_experiments}.]
    \end{enumerate}
    
    \item Does this paper rely on one or more datasets? [Yes.]
    \begin{enumerate}
        \item A motivation is given for why the experiments are conducted on the selected datasets 
        [Yes.]
        \item All novel datasets introduced in this paper are included in a data appendix. 
        [Yes.]
        \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. 
        [NA. All datasets used in this paper are publicly available.]
        \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. 
        [Yes.]
        \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. 
        [Yes.]
        \item
        All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. 
        [NA. All datasets used in this paper are publicly available.]
    \end{enumerate}
    
    \item Does this paper include computational experiments? [Yes.]
    \begin{enumerate}
        \item Any code required for pre-processing data is included in the appendix. 
        [Yes. Details for dataset split are disclosed in Appendix \ref{sec:append_experiments}.]
        \item All source code required for conducting and analyzing the experiments is included in a code appendix. 
        [NA. The code will be released after publication.]
        \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. [Yes.]
        \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from
        [Yes.]
        \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. [Yes.]
        \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. [Yes, see Appendix \ref{sec:append_experiments}.]
        \tiem This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. [Yes, see Appendix \ref{sec:append_experiments}.]
        \item This paper states the number of algorithm runs used to compute each reported result. [Yes.]
        \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. [No.]
        \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). [No.]
        \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. [Yes.]
        \item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. [Yes.]
    \end{enumerate}
    

\end{enumerate}













==> cover_letter.tex <==
\newpage
\section{Cover Letter (NeurIPS-22 submission)}
\subsection{Changes made since the NeurIPS-22}
Per the NeuIPS reviewers' comments and suggestions, 
we modify the submission and further report some additional experimental results. 
\begin{enumerate}[leftmargin=*]
    \item We revise the theoretical analysis in Sec. \ref{sec:analysis} to connect it more explicitly to the other parts of the paper (e.g., using the same notation, more explanations).
    \item We discuss the reasons conducting stronger white-box attacks instead of black-box attacks on Sec. \ref{sec:analysis}.
    \item We adopt Adversarial Training as a new baseline, as suggested by a NeurIPS reviewer. Details can be found in Appendix \ref{sec:append_experiments}.
    \item We measure the correlation between thickness and the P@k metric on the model-level to explore the tight relationship between these two metrics.
    The experimental results are shown on Sec. \ref{sec:experiemnt_whole_section} and Appendix \ref{sec:append_experiments}.
    \item As the gradient-based explanation methods, we not only consider SimpleGrad, but also IntegratedGradient and SmoothGrad. The corresponding results are disclosed on Appendix \ref{sec:append_experiments}, and similar conclusions to SimpleGrad in Sec. \ref{sec:experiemnt_whole_section} can be drawn.
    \item We evaluate the explanation faithfulness by three widely used metrics, including DFFOT, COMP and SUFF. 
    The experimental results are disclosed on Appendix \ref{sec:append_experiments}.
    \item Note that the review ``ERAttack does not constrain the prediction'' is incorrect, since we conduct both ERAttack and MSE attack by constrained optimization algorithms, which retains the target model's predictions unchanged.
    More details are disclosed in Appendix \ref{sec:append_experiments}.
    \item We correct most typos in the submission.
\end{enumerate}


\subsection{Rebuttal for NeurIPS reviewers}
Concerning the NeurIPS reviewers' comments and reviews, 
we have the following rebuttals and feedback.
\begin{itemize}[leftmargin=*]
    \item Address Official Reviews by Reviewer \textit{Y1j2}.
    
    Concerning the comments on the ``Strengths And Weaknesses'':
    We admit that the problem of explanation robustness has been explored recently. However, prior work mainly focused on the effects of gradient or Hessian norm smoothing on robustness, which we proved to be only marginally relevant. We provide a new perspective instead, revealing the connection between the robustness of explanation and thickness with theoretical analysis. Algorithmically, we proved bounds to avoid the computational cumbersome integration and make robust explanations practical.

    Concerning the questions:
    We appreciate the suggestions regarding the paper organization and will take care of them in the camera-ready version. The limited human attention capacity is to motivate the ranking-based explanation, since human users can attend only to the top-ranked salient features. That further motivates the robustness of the ranking-based explanations and thus the thickness of the explanations. Future work will address the weaknesses that we admitted in the conclusion.
    
    \item Address Official Reviews by Reviewer \textit{KSdW}.
    
    Concerning the comments on the ``Strengths And Weaknesses'':
    To clarify, R2ET works during the training phase of a model, aiming to generate an accurate model that can be robustly explained. IntegratedGradient and SmoothGrad are post-hoc explanation methods that work on a fixed trained model and do not smooth the gradient/Hessian during training time. In other words, both IntegratedGradient and SmoothGrad play the same role as the simple gradient-based explanation method adopted by the submission. It is, therefore, more appropriate to compare the robustness of explanations of models trained with and without R2ET, generated by gradient-based explanation methods (e.g., IntegratedGradient or SmoothGrad). We added these comparisons in Table 5 in Appendix D and find that R2ET always improve the robustness, whether the explanations are generated by simple Gradient, IntegratedGradient, or SmoothGrad.

    Concerning the questions in the list:
    \begin{enumerate}
        \item ``I understand what you are trying to convey in Figure 1, but as far as I can tell, in both cases,  $I(x^\prime)-I(x)$ seems to be larger because the norm of $I(x^\prime)$ is larger! Perhaps this is not a good illustration of your argument.''
        
        A1. We believe that you are discussing the norm of $I(x^\prime)-I(x)$, since $I(x^\prime)-I(x)$ is a vector and cannot be compared with another vector. We could have used an $I(x^\prime)$ with all saliency scores much smaller than those in $I(x)$ to induce a large gap $|I(x^\prime)-I(x)|$, with the same feature ranking in $I(x^\prime)$. As a result, the norm of $I(x^\prime)$ is not relevant. Feature ranking is a relative quantity and the norm of saliency scores is an absolute quantity.
        
        \item
        ``Instead of ranking thickness, wouldn't an $\ell_p$-norm of $p\approx 1$ be a better compromise, as unlike ranking thickness $\Theta$, it is continuous?''

        A2. It is unclear to us which vector's $\ell_p$ norm the comment referred to. Figure 1 already shows that the norm $|I(x^\prime)-I(x)|$ is not indicative of the difference in feature rankings and is irrelevant to ranking-based explanation robustness.
        
        \item
        ``Isn't $\delta=0$ the optimal solution of (1)? :)''

        A3. There is a typo in Eq. (1) and the min operator should have been the max operator, since the adversary wants to maximally perturb the explanation $I(x)$ to a different one. As a result, $\delta=0$ will not do any perturbation.
        
        \item
        ``Isn't the observation in Lines 114 and 115 (second-order back-propagation) applicable to the loss in (5) as well?''

        A4. We do not attempt to bypass the computations and evaluations of $I(x)_i-I(x)_j$ mentioned in line 114 and 115. Rather we use the second term in Eq. (5) to address the cost associated with the expectation and integration in Eqs. (2) and (3). In Eqs. (2) and (3), if we evaluate $\Theta$ using Monte Carlo sampling for the expectation and integration operators, and if it needs $M_1$ samples of  and $M_2$ samples for interpolation, then we have the cost of backward propagation multiplied by $2\times M_1 \times M_2$ for each $x_r$. On the contrary, using the surrogate in Eq. (5), we avoid the expectation and integration and only 2 backward propagations are needed for each $x_r$.
        
        \item
        ``L 125: In the Appendix, I was unable to find the bounds for the local ranking thickness (Definition 3.2). Is it not possible to minimize a bound on this quantity instead of a bound on its relaxed version?''

        A5. The proof of the bounds for the local top-$k$ ranking thickness is given at the end of Appendix B.
        
        \item
        ``It is quite difficult to appreciate Section 4. For example: What is $\theta$ in (6)? In Thm 1, what is the significance of Fmin and Fmax? They appear to be irrelevant. Overall, this section appears to be quite disconnected from the rest of the paper.''

        A6. 1) $\theta$ was a typo and should have been $\bw$, which is the parameter of the model of $f$. 
        2) $F_{\textnormal{max}}$ is the maximal value of any thickness term in Eq. (5) and $F_{\textnormal{min}}$ is the minimal value of the terms. Intuitively, the larger the individual thickness terms (represented by a large gap in $F_{\textnormal{max}} -F_{\textnormal{min}}$), the more iterations are needed for the attacking algorithm ERAttack to successfully alter any pair of salient and non-salient features in the ranking-based explanation. The theory is confirmed by the first and third subfigures of Figure 2. Analyzing the convergence of the overall sum of all the thickness terms (which is a scalar) is less meaningful for the attacker as a small sum does not necessarily indicate any successful flipping of salient/non-salient features. Multiple thickness terms become a vector in Eq. (6) and the multi-objective analysis is necessary.
        
        \item
        ``Constant functions are the most robust, but they are useless! Can you ensure that R2ET does not adversely affect the quality of explanations? R2ET might appear to be more robust, but its explanation quality may actually be lower. Any evidence beyond the visual inspection of Section 5.4?''

        A7. This question has two parts: 1) we agree that R2ET should not promote explanation robustness at the cost of generating a constant function. R2ET trains models with similar high AUC as the original models and thus the models cannot be constant functions. 2) There are several explanation quality metrics, including visual evidence, faithfulness, and robustness. We already showed improved robustness and visual evidence in the original submission. Note that faithfulness is evaluated against a particular model, and a model generated by R2ET should have a different explanation than the explanation of another model (thus the faithfulness). It is thus unreasonable to compare two explanations of two different models. Rather, one should compare an explanation against the associated model for evaluating faithfulness. In Table 6 in Appendix D, we added new results of faithfulness.
        
        \item
        ``Another question related to this is how does R2ET affect the performance of the model for the original task it was trained for?''

        A8. R2ET trains models that are accurate in prediction, thanks to the first objective function of Eq. (5). Similar high AUCs are reported in Appendix C.4.2. Other baselines represent other training procedures that can lead to high accuracy but low explanation robustness.

        \item 
        ``Is there any particular reason why you did not consider common classifiers trained on MNIST and CIFAR-10?''

        A9. We do have the CNN architecture on MNIST, with a contrastive loss (due to the Siamese network) for the training. The current experiments have firmly proved our hypotheses and theoretical analyses. We can add experiments on CIFAR-10 in an extended version.

        \item 
        ``ERAttack does not constrain the prediction, and it may alter it. In such as case, why should we expect the same top-k features to be still relevant if the prediction changes?''

        A10. We do have constraints to ensure that ERAttack does not alter the original predictions, using constrained or multi-objective optimization algorithms, including Gradient Descent Ascent (GDA), Hedge, and Quadratic Programming (QP) (see Appendix C.5.4). As a result, all the reported attacks have similar AUC before and after the attacks (see Appendix C.5.5.) Note that on MNIST, R2ET achieved the original high AUC (ranging from 0.98 to 0.99) without the constraints. We admit that there is a presentation issue, that we did not explicitly mention the accuracy constraints in ERAttack.

        \item
        ``Instead of SSR, you could use standard  $\ell_\textnormal{inf}(\ell_2)$ adverasrial training since they seem to have a similar smoothing effect. I would recommend adding it to Table 1 as a baseline. On all datasets you considered, it should not be too difficult to obtain adversarially trained models.''

        A11. Adversarial training is not scalable due to solving an optimization problem in each iteration of model training. Authors of [25] demonstrated the connection between Adversarial Training and the smoothing of the Hessian, and used the Hessian norm as a surrogate regularization to achieve performance (clean and adversarial accuracy) similar to adversarial training. Note that [25] targets at robust model predictions rather than explanations. We added the results of adversarial training in the latest supplementary (Appendix D.1) .

        \item 
        It would be useful to demonstrate the effectiveness of R2ET using a stronger adversary targeting directly $\Theta$ or P@k. Evolutionary attacks may be useful in this regard.

        A12. Both ERAttack and MSE are white-box attacks and should represent the strongest attacks, compared to black- or grey-box attacks. ERAttack attempts to flip the ranking positions of the salient and non-salient features by directly minimizing $\sum_i \sum_j h(x_r,i,j)$. 
        See line 220 and Appendix C.5.1. $\Theta$ has the indicator function and is thus not differentiable. We prove $\sum_i \sum_j h(x_r,i,j)$ can be used to bound  $\Theta$ and attacking $\sum_i \sum_j h(x_r,i,j)$ is reasonable. P@$k$ is non-differentiable.

        \item 
        ``It may be useful to report the explanation thickness  $\Theta$ for the models in Table 1 to see how well the conclusion of Section 5.3 applies to these models.''

        A13. In Table 7 in Appendix D, we report the thickness for all models. The model with higher explanation thickness usually performs better concerning P@$k$ metric.

        \item
        ``What are the ground truths for “important features”?''

        A14. Pixels defining the digits can be regarded as ground truth (MNIST). The remaining pixels are considered unimportant. Figure 3 shows that R2ET and R2ETmm can focus on some of the ground truth important features as explanations, while the baseline explanations scatter around both salient and non-salient ones.
        
    \end{enumerate}

    \item Address Official Reviews by Reviewer \textit{8Jmi}.

    Concerning the weakness 1, we have four main arguments.
    \begin{enumerate}
        \item Since humans can process only a small number of important features based on psychology research, selecting the top few salient features helps humans make sense of the prediction. Admittedly, the saliency scores are useful, but without important features ranked at the top in the first place, saliency scores that fail to highlight important features are actually misleading.
        \item Given the same salient feature ranking, the underlying saliency intensity can of course be different but can be visualized and inspected by humans, as shown in Figure 3.
        \item Saliency scores are defined with respect to the triple of (model, input, explanation-method). So long as the scores are well-defined and can be computed with good enough accuracy against the triple, there is no loss of saliency information.
        \item Based on visual inspection of Figure 3, there is no evidence that R2ET makes the saliency intensity inaccurate given the superior feature ranking, and R2ET's saliency scores range similar to those of other baselines (Vanilla and WD).
    \end{enumerate}
    
Concerning the weakness 2:
We deliberately chose the two white-box attacks (ERAttack and MSE) to show that R2ET is sufficiently robust to withstand attacks on the stronger side. It is unlikely that black-box attacks will achieve the same level of attack strengths given the same amount of computation resources, as it is widely recorded that black-box attacks are weaker than white-box attacks. Besides, the AAAI-22 paper by Fang S and Choromanska A proposes a backdoor attack occurring during training, while ERAttack aims to perturb the explanation.

Concerning the weakness 3:
We are aware of robust ranking in IR and we cited these papers [51] in our submission. There are several key differences between ranking robustness in IR and in explanations.
\begin{enumerate}
    \item the vulnerabilities are different. IR has queries and candidates that can be attacked, while we focus on attacking the gradient of classifiers via input manipulation.
    \item the attacking objectives are different. In IR [51], authors either manipulate the ranking of one single candidate, or manipulate query to distort the ranking of candidates. In this paper, we aim to swap any pair of salient and non-salient features and we do not find a similar goal in IR papers.
    \item the computations are different. Explanations are defined by gradient or its variants and studying their robustness requires second- or higher order derivatives. The cost of higher-order derivatives requires us to design a surrogate regularizer to bypass the costly computations. These challenges are less seen in IR.
\end{enumerate}


Concerning the weakness 4:
We assume the referred paper is titled ``Improving Deep Learning Interpretability by Saliency Guided Training''. Algorithmically, they create a perturbed input $x^\prime$ by masking the k least important features for each input $x$, and add KL($x, x^\prime$) into the objective function. First of all, this paper is not designed to improve the robustness of explanations, but to improve the faithfulness of gradient-based explanations due to noise, which differs from our goal. Correspondingly, they do not show the performance of explanation robustness under attacks. Second, they perturb the inputs by masking out the least important features by gradient rankings, while we show that gradient rankings from vanilla models can be vulnerable and misleading.

Concerning Questions:
\begin{enumerate}
    \item ``have you examined the distribution of the saliency, particularly in natural images, to see if it is indeed multi-modal where rank-based approach may perform better?''
    
    A1. The reason that our ranking-based approach works better is not that the saliency scores are multi-modal. Rather, our theory in Section 4 shows that it takes more optimization iterations to alter the ranking if the gap between salient and non-salient features is large.

    \item ``have you tried black-box attacks of explanation?''

    A2. White-box attacks, such as ERAttack and MSE attacks, are stronger than black-box attacks. Besides, black-box attacks need to evaluate the model's explanations (not predictions) multiple times and thus may not be practical for the attackers. In particular, an attacker has to query multiple salient maps multiple times for iterative optimization, and such behaviors can be detected by the defender.
\end{enumerate}

Responses to the concerns in the ``Limitations'':

Our main contribution is to design a theoretically sound defense of explanation against strong attacks. Our main (surprising) finding is that previous widely used smoothing-based approaches do not help explanation robustness. Evaluating the proposed theory and techniques on natural images can be considered as an application of this work and will add more practical value rather than the theoretical value. On the other hand, we have confirmed our theory on tabular, image, and graph datasets with three different neural network architectures (MLP, CNN, and GNN). Due to the diverse data formats and network architectures, we have high confidence that our theory can generalize to natural images well.

    \item Address Official Reviews by Reviewer \textit{hUB4}.
    Respond to comments on the ``Strengths And Weaknesses'':
    \begin{enumerate}
        \item 
        We motivate the design of the objective function (thickness) for robust explanation in Eq. (2) by the manipulability of the gradients of a model. Prior work showed that the network architecture, especially the activation functions, also has a significant impact on the explanation robustness. There is no strict separation of these two factors (gradient vs. network arch) in the prior since they are used in two different stages (model explaining vs. design). Our experiments show that the gradient-based explanations of three neural network architectures, including MLP, CNN, and GNN, lack robustness. Unlike prior work that focuses on robustness due to explanation algorithms and network architecture, our work shows that the training objective function (Eq. (5)) can obtain network parameters that contribute to the robustness of explanations of the trained models.
        
        \item 
        The main contribution of this work is the theoretically motivated algorithms and the surprising contrast with previous smoothing methods that were believed to improve explanation robustness. Evaluating the methods on large-scale image datasets would be of practical interest but not contribute to our theoretical aspects of the work, and thus not included. We can include that in an extended version of the work. All of our datasets are collected from the real-world (e.g., the BP and ADHD datasets are from medical experiments) and not toy datasets. On the other hand, the diversity of the data format (tabular, graph, and image) and network architecture (MLP, GNN, and CNN) demonstrates the generality of the proposed approach.

        \item
        We evaluate the faithfulness of all the models by three widely used metrics, and report the corresponding results in Table 6 in Appendix D.

    \end{enumerate}

To address the questions:

\begin{enumerate}
    \item 
    A motivating application of explanation robustness: Alice applied for a student loan from a bank but the application was rejected by a machine learning model used by the bank, and the explanation was "low credit score''. One month later, she tried again with only a slightly higher score which is not significant to get the application through (everything else is the same). The same model rejected her application again, but this time the explanation was changed to "the gender is not male''. The two explanations would have been better if they consistently gave ``low credit score'' as the reason for both the rejections. The inconsistency in explanations due to slight credit score change is not desirable and we aim to train models are can give consistent explanations even with slight input perturbations. There are other applications of machine learning to the medical domain where doctors need consistent explanations.
    
    \item In Table 6 of Appendix D, we include additional evaluations of faithfulness metrics to show that our method achieves a similar level of faithfulness as the baselines. We conclude that robust explanations do not affect explanation faithfulness.

\end{enumerate}


\end{itemize}
    

==> defender.tex <==
\section{Defender}

Existing works make the explanations more robust by retraining the target model by fine-tuning the model structure \cite{dombrowski2019explanations,dombrowski2021towards}, training with adversarial samples \cite{madry2017towards} or adding smoothing regularizers \cite{dombrowski2021towards,wang2020smoothed,moosavi2019robustness}.
We focus on adding smoothing regularizers for robustness.

\subsection{Hessian-Free Smoothing}
\label{sec:hvp}
A strategy for more robust explanations is smoothing the target model's curvature,
which can be depicted by the Hessian matrix $H$ \cite{moosavi2019robustness,dombrowski2021towards}.
The Hessian of a function $f(x)$ with respect to a $d$-dim input $\mathbf{x}$ is defined by
\begin{equation}
    \label{eq:definition_hessian}
    H = 
    \left( \frac{\partial^2 f}{\partial \mathbf{x}_{[i]} \mathbf{x}_{[j]}} \right)
    \in\mathbb{R}^{d\times d},
\end{equation}
where $\mathbf{x}_{[i]}$ denotes the $i$-th entry of $\mathbf{x}$.
Due to the heavy calculation of Hessian matrix,
recent researches \cite{moosavi2019robustness,pearlmutter1994fast} apply 
% the Pearlmutter's trick, 
a Hessian-free method to compute the multiplication of the Hessian matrix and any vector $\mathbf{v}$ as
% The Hessian vector products can be given by the finite difference
\begin{equation}
    \label{eq:hessian_vector_product_fd}
    H\mathbf{v} = \lim_{h\to0} \frac{\nabla f(\mathbf{x}+h\mathbf{v}) - \nabla f(\mathbf{x})}{h}
    \approx \frac{\nabla f(\mathbf{x}+h\mathbf{v}) - \nabla f(\mathbf{x})}{h}.
\end{equation}
In practice, 
$H\mathbf{v}$ is estimated by assigning $h$ as a small value.
Furthermore, 
a model with smoother curvature can be trained by adding Hessian-related penalty term to all training samples 
% one can apply a new objective function to all training samples to train a robuster model 
\cite{moosavi2019robustness,dombrowski2021towards} as
\begin{equation}
    \label{eq:robust_obj}
    \mathcal{L} = 
    % \frac{1}{|\textnormal{Tr}|} \sum_{i\in\textnormal{Tr}} 
    % (
    \mathcal{L}_{ord} + \alpha \mathcal{L}_H,
    % ), 
    \quad \quad \quad
    \textnormal{where }
    \mathcal{L}_H = \|H\mathbf{v}\|^2,
\end{equation}
where $\alpha$ is a balancing weight
and $\mathcal{L}_{ord}$ is the original classification loss.

\subsection{Rethink Smoothing Regularizer}
The robustness enhanced objective function, 
Eq. (\ref{eq:robust_obj}),
is applied to \textit{all} training data samples by default in existing works \cite{moosavi2019robustness,dombrowski2021towards}.
As a result,
the accuracy of the robustness enhanced models is usually significantly worse than the vanilla models'.
However,
we argue that there is a chance to improve the robustness without sacrificing accuracy much.
The key intuition is to add robustness regularizer selectively rather than indiscriminately.

% \begin{figure}
%     \centering
%     \begin{minipage}[c]{\textwidth}
%     \centering
%     \includegraphics[width=3.0in]{figs/eight-case.pdf}
%     \caption{Caption for image}
%     \label{fig:sample_figure}
% \end{minipage}
% \end{figure}

\begin{figure}
      \centering
      \begin{minipage}{0.45\textwidth}
        %   \includegraphics[width=\textwidth]{figs/eight-case.pdf}
        %   \caption{This is the second figure}
        \centering
        \begin{tabular}[b]{c|c|c|c}
        \toprule
        \multirow{2}{*}{Prediction} &
        \multirow{2}{*}{Sensitivity} &
        \multicolumn{2}{c}{Curvature}
        \\
        \cline{3-4}
        & & Low & High \\ 
        \hline
        \multirow{2}{*}{Correct} & No & \circled{1} & \circled{2} \\
        \cline{2-4}
        & Yes & \circled{3} & \circled{4} \\
        \hline
        \multirow{2}{*}{Incorrect} & No & \circled{5} & \circled{6} \\
        \cline{2-4}
        & Yes & \circled{7} & \circled{8} \\
        \bottomrule
        \end{tabular}
        \caption{\small
        Depending on the prediction, sensitivity of and curvature around the sample,
        we can specify eight different cases.}
        \label{fig:eight-case-table}
      \end{minipage}
      \hspace{0.05\textwidth}
      \begin{minipage}{0.45\textwidth}
          \includegraphics[width=\textwidth]{figs/eight-case.pdf}
          \caption{\small 
          A toy example shows a positive sample in eight cases geometrically.
          \textcolor{red}{What is confusing is the mix-up of the decision boundary and the more general level sets. The solid black curve is the boundary but there are other level sets where gradient-based explanations can be attacked easily.}}
        \label{fig:eight-case-geometry}
      \end{minipage}
\end{figure}

As shown in Figure \ref{fig:eight-case-table},
each sample can either locate in one of eight different regions depending on 
whether the prediction of the sample is correctly classified,
whether the sample is closed to decision boundary (sensitivity of prediction),
and whether the curvature around the sample is low.
Figure \ref{fig:eight-case-geometry} shows a toy example for a positive sample,
where the black curve is the model's decision boundary,
and sensitive samples sit on the (small) region between two yellow dash curves.
Previous works \cite{moosavi2019robustness} lower
the curvature around every sample no matter where the sample locates,
and it easily raises the conflicts between accuracy and robustness.
Take sample in case-3 in Figure \ref{fig:eight-case-geometry} as a counterexample,
the green dotted line makes the curvature slightly smaller 
(where a line with zero curvature),
while the prediction is flipped to wrong class due to improper linearity around the sample.
On the contrary,
an ``acceptable'' trade-off between accuracy and robustness should occur in the case-4 (and maybe case-2),
which means the prediction is misled while the robustness is significantly improved from black curve to the red dashed one.
A ``free lunch'' to train a robuster model is to lower the curvature around the samples in case-8 and case-6, 
which benefits both accuracy and robustness.
An example is to flatten the curvature around samples in case-8 to purple dashed curve, 
where the predictions of the samples are corrected simultaneously.

\textcolor{red}{Need an algorithm description here for the re-training algorithm.}
